3D Video Object Detection with Learnable Object-Centric Global Optimization

We explore long-term temporal visual correspondence-based optimization for 3D video object detection in this work. Visual correspondence refers to one-to-one mappings for pixels across multiple images. Correspondence-based optimization is the cornerstone for 3D scene reconstruction but is less studied in 3D video object detection, because moving objects violate multi-view geometry constraints and are treated as outliers during scene reconstruction. We address this issue by treating objects as first-class citizens during correspondence-based optimization. In this work, we propose BA-Det, an end-to-end optimizable object detector with object-centric temporal correspondence learning and featuremetric object bundle adjustment. Empirically, we verify the effectiveness and efficiency of BA-Det for multiple baseline 3D detectors under various setups. Our BA-Det achieves SOTA performance on the large-scale Waymo Open Dataset (WOD) with only marginal computation cost. Our code is available at https://github.com/jiaweihe1996/BA-Det.

==> tables/ba_params.tex <==
% \begin{table*}
% \begin{minipage}{0.4\linewidth}
%  \centering
% \caption{Table 1} 
% \begin{tabular}{l|cccc}
% \toprule
% 3D AP$_\text{70}$ & 3D APH$_\text{70}$ & 3D AP$_\text{50}$ & 3D APH$_\text{50}$\\
% \midrule

% \bottomrule
% \end{tabular}
% \end{minipage}
% \begin{minipage}{0.4\linewidth}
%  \centering
% \caption{Table 1}
% \begin{tabular}{l|cccc}
% \toprule
% 3D AP$_\text{70}$ & 3D APH$_\text{70}$ & 3D AP$_\text{50}$ & 3D APH$_\text{50}$\\
% \midrule

% \bottomrule
% \end{tabular}
% \end{minipage}
% \end{table*}

 \begin{table}[]
 \begin{minipage}{0.45\linewidth} 
 \centering 
 \caption{\textbf{Parameters of bundle adjustment.}} 
 \resizebox{\linewidth}{!}{
 \begin{tabular}{l|cccc}
\toprule
3D AP$_\text{70}$ & 3D APH$_\text{70}$ & 3D AP$_\text{50}$ & 3D APH$_\text{50}$\\
\midrule
\bottomrule
\end{tabular}}
\end{minipage} 
\hfill
\begin{minipage}{0.45\linewidth} 
\centering 
\caption{\textbf{Parameters of bundle adjustment.}}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
3D AP$_\text{70}$ & 3D APH$_\text{70}$ & 3D AP$_\text{50}$ & 3D APH$_\text{50}$\\
\midrule
\bottomrule
\end{tabular} }
\end{minipage}
\end{table} 

==> tables/oracle.tex <==
\begin{table}[h]
\caption{\textbf{Oracle experiments.}}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|cccc}
\toprule
&\multicolumn{4}{c|}{LEVEL\_1} 
&\multicolumn{4}{c}{LEVEL\_2} \\
& 3D AP$_\text{70}$ & 3D APH$_\text{70}$ & 3D AP$_\text{50}$ & 3D APH$_\text{50}$ & 3D AP$_\text{70}$ & 3D APH$_\text{70}$ & 3D AP$_\text{50}$ & 3D APH$_\text{50}$ \\
\midrule
w/ gt correspondence &\\
w/ gt \\
\midrule
\textcolor{gray}{optimization upper bound}\\

\bottomrule
\end{tabular}}
\label{tab:oracle}
\end{table}
